Extending the Epoch of Reionization window with apt Foreground and Instrument modeling

It is seen that foregrounds of 21cm Epoch of Reionization experiments, which are expected to have smooth spectral dependence, are dominant in a wedge shaped region of the Fourier space called as Foreground Wedge. A possible way forward to isolate the 21cm Epoch of Reionization (EoR) signal from the much larger foreground component is to focus on the remaining portion of the Fourier space called as the EoR window. There are in-fact three distinct regions in the Fourier space, (i) the Foreground wedge portion, (ii) the EoR window region which lies beyond Horizon wedge and (iii) the region in between the Horizon wedge and the Field of View wedge. This paper addresses two questions: (1) Whether the signal in between the two wedges is also a direct representation of the EoR brightness temperature fluctuations? and (2) How can we extract the cosmology information from this region considering that the foregrounds are much larger than the signal? The answer to the first question is yes, the visibilities as function of baseline and delay are, within a few percent, same as the EoR brightness temperature fluctuations for the cases considered. Secondly, the in between region is not foreground free, due to non-negligible sidelobes. But, one can possibly extract signal from this region if one models foregrounds and instruments accurately. As all the three components, the cosmological signal, the foregrounds and the thermal noise are calculated in the same space, the analysis suggested could be more straightforward.

==> adsbib3 <==
#!/usr/bin/perl

$aux = ($#ARGV >= 0) ? "$ARGV[0]" : "ms";
$bib = ($#ARGV >= 1) ? "$ARGV[1]" : $aux;

print "`adsbib` is creating a BibTeX database for \"$aux.tex\":\n";

open AUX, "< $aux.aux";
while (<AUX>) {
    if ($_ =~ m/\\citation\{/i) {
	foreach (split(',', substr($_, 10, -2))) {
	    push @code, $_
		if $_ =~ m/(\d{4}\D\S{13}[A-Z.:])/i;
	}
    }
}
close AUX;

use List::MoreUtils qw/ uniq /;
@ucode = uniq sort @code;

$count = 0;
foreach (@ucode) {
    if (system("grep '\{$_,' my.bib 2> /dev/null")) {
	printf "%4d. %s\n", ++$count, $_;
    } else {
	splice @ucode, $count, 1;
   }
}

$server = 'adsabs.harvard.edu';
$script = 'cgi-bin/nph-bib_query';
$opt{data_type}   = 'BIBTEX';
$opt{db_key}      = 'ALL';
$opt{nocookieset} = '1';

$url  = "http://$server/$script?";
$url .= "$_=$opt{$_}&" foreach keys %opt;
$url .= "bibcode=";
$url .= "$_&" foreach @ucode;

use LWP::Simple;
$all = get $url;
die "ERROR: Couldn't get bibTeX data\n" unless defined $all;
@line = split('\n', $all);

open BIB, "> $bib.bib";
$head = '% ';
foreach (@line) {
    $_ =~ s/\ \&/\ \\and/g;
    print BIB "$head$_\n";
    if ($_ =~ m/^Retrieved/) {
	$head = '';
    }
}
close BIB;

